Synthesizing Min-Max Control Barrier Functions For Switched Affine Systems

We study the problem of synthesizing non-smooth control barrier functions (CBFs) for continuous-time switched affine systems. Switched affine systems are defined by a set of affine dynamical modes, wherein the control consists of a state-based switching signal that determines the current operating mode. The control barrier functions seek to maintain the system state inside a control invariant set that excludes a given set of unsafe states. We consider CBFs that take the form of pointwise minima and maxima over a finite set of affine functions. Our approach uses ideas from nonsmooth analysis to formulate conditions for min- and max- affine control barrier functions. We show how a feedback switching law can be extracted from a given CBF. Next, we show how to automate the process of synthesizing CBFs given a system description through a tree-search algorithm inspired by branch-and-cut methods from combinatorial optimization. Finally, we demonstrate our approach on a series of interesting examples of switched affine systems.

==> tree-search-old.tex <==



Following Def.~\ref{def:polyhedral-cbf}, we require that the control barrier function must satisfy conditions \textbf{(C1)-(C3)}. We first focus on encoding \textbf{(C1)} and \textbf{(C2)}. 
\[ \mathbf{(C1):}\ \forall\ x \in X_0,\ B(x) < 0,\   \mathbf{(C2):}\ \forall\ x \in X_u,\ B(x) > 0 \,.\]
Let $\epsilon_0 > 0$ be a fixed constant threshold. It is sufficient to find $(c_i, d_i)_{i=1}^k$ such that: 
\[ \mathbf{(D1):}\ \forall\ x \in X_0,\ B(x) \leq -\epsilon_0,\  \mathbf{(D2):}\ \forall\ x \in X_u,\ B(x) \geq \epsilon_0 \,.\]
Note that  \textbf{(D1)} can be equivalently written as $ \forall x \in X_0,\ \bigwedge_{i=1}^k c_i^t x - d_i \leq -\epsilon_0$. This can be converted into a constraint involving $c_i, d_i$ using Farkas' lemma.

\begin{thm}[Farkas Lemma]
Let $X$ be a nonempty polyhedral set denoted by the constraint $A x \leq b$. 
The assertion $\forall x \in X, c^t x \leq d $ holds iff there exists multipliers $y \geq 0$ such that 
$ A^t y = c,\ b^t y \leq d,\ y \geq 0$.
\end{thm}

Let $P_0 x \leq q_0$ denote the constraint representation of $X_0$. 
Therefore, \textbf{(D1)} can be written equivalently as a condition $\psi_1$ involving $(c_i, d_i)_{i=1}^k$ and vectors of multipliers $y_1, \cdots, y_k$:
\begin{equation}\label{eq:d1-prime}
\psi_1\ := \ \left( \bigwedge_{i=1}^k\ P_0^t y_i = c_i\ \land\  q_0^t y_i \leq d_i - \epsilon_0\ \land\  y_i \geq 0 \right) \,. 
\end{equation}
$\psi_1$ is a conjunction of linear equalities/inequalities involving $(c_i, d_i)_{i \in [k]}$ and multipliers $y_1, \ldots, y_k$.

Next, we focus on \textbf{(D2)} that enforces $\forall x \in X_u,\ B(x) \geq \epsilon$. Note that $\max_{i=1}^k c_i^t x - d_i \geq \epsilon$ iff $\bigvee_{i=1}^k c_i^t x - d_i \geq \epsilon$. As such this is a disjunction of linear inequalities and does not yield a polyhedron. However, the two convex sets $X_0, X_u$ do not intersect. By the separating hyperplane theorem, there must be a hyperplane $p^t x - q \leq 0$ such that $\forall x \in X_0, p^t x \leq q$ and forall $x \in X_u$, $p^tx > q$. 
We will force the first piece $c_1^t x - d_1 \leq 0$ to serve as this separating hyperplane: i.e,  $\forall\ x \in X_u, c_1^t x - d_1 \geq \epsilon_0$. Let $P_u x \leq q_u$ denote the polyhedral representation of $X_u$. Applying Farkas' lemma, we obtain the conditions:
\begin{equation}\label{eq:d2-prime}
\psi_2:= \left(  P_u^t z = -c_1\ \land\ q_u^t z \leq -d_1 -\epsilon_0 \ \land\  z \geq 0  \right) \,.
\end{equation}

\begin{comment}
\begin{rem}
    Considering the point-wise minimum function as a barrier certificate, the condition \textbf{(C1)} and \textbf{(C2)} is encoded as \textbf{(E1)} and \textbf{(E2)}, respectively. 
    \[\textbf{(E1):} \forall x \in X_0, \bigvee_{i=1}^k c_i^t x - d_i \leq -\epsilon_0,\]
    \[\textbf{(E2):} \forall x \in X_u, \bigwedge_{i=1}^k c_i^t x - d_i \geq \epsilon_0.\]
\end{rem}
\end{comment}

\subsection{Tree Search Algorithm}
Let $C_0: \psi_0\ \land\ \psi_1 \ \land\ \psi_2$ represent the set of all coefficients $(c_i, d_i)_{i=1}^k$ satisfying ~\eqref{eq:cd-bounds}, ~\eqref{eq:d1-prime} and~\eqref{eq:d2-prime}. This is a polyhedral constraint over the coefficients and some multiplier vectors $y_1, \ldots, y_k$, and $z$. 

The tree search algorithm maintains a tree $T$,  wherein each node $n_j$ of the tree is labeled with a polyhedral constraint over the coefficients $(c_i, d_i)_{i=1}^k$.  Let $C(n_j)$ denote the constraints associated with node $n_j$. 

The root node of the tree $n_0$ is labeled with the constraint $C(n_0) = C_0$. For each non-root node $n$ with parent node $p$, we will satisfy the relation:
$ C(n) \subset C(p)$. 

Each iteration of the algorithm proceeds as follows:
\begin{enumerate}
\item Pick a previously unexplored leaf node of the tree $n$. Mark it as explored.
\item Pick a candidate solution $B(x) = \max_{i=1}^k \hatc_i^t x - \hatd_i $ such that $(\hatc_i, \hatd_i)_{i=1}^k \in C(n)$.
\item \textbf{Verify} condition \textbf{(C3)} for $B(x)$:
\begin{enumerate}
\item If \textbf{(C3)} is verified successfully, then return $B(x)$ as the control barrier function. 
\item Otherwise, we obtain a counterexample point $x_c$ that fails to satisfy \textbf{(C3)}.
\item Use the counterexample $x_c$ to \textbf{expand the node} $n$ by adding new children $n_1, \ldots, n_j$ and their corresponding polyhedra $C(n_1), \ldots, C(n_j) \subseteq C(n)$. 
\end{enumerate} 
\end{enumerate}

\subsection{Verification Procedure}

We will now describe the procedures for verifying condition \textbf{(C3)} given a barrier function candidate $B(x) = \max_{i=1}^k \hatc_i^t x - \hatd_i$ or finding a counterexample $x_c$. We will focus on solving for a counterexample $x_c$ as a mixed-integer linear program (MILP). Infeasiblity of this MILP will signal that $B(x)$ is a valid CBF.

First, we enforce that $\max_{i=1}^k \hatc_i^t x_c - \hatd_i \leq 0$.
Furthermore, we require that $x_c$ must violate \textbf{(C3)} for $B(x)\leq 0$. So, the logical negation of \textbf{(C3)}, which is written as:
\begin{equation}\label{eq:counterex-eq}
\forall\ l \in [m],\ \exists\ i \in [k],\ \left( \begin{array}{c}
\hatc_i^t x_c - \hatd_i \leq 0\ \land\\
\bigwedge_{j=1}^k \hatc_i^t x_c - \hatd_i \geq \hatc_j^t x_c - \hatd_j\ \land\\
\hatc_i^t (A_l x_c + b_l) \textcolor{red}{\geq} -\lambda (\hatc_i^t x_c - \hatd_i) \end{array} \right) \,.
\end{equation}
Note that the constraint requires us to map each $l \in [m]$ to a piece $i \in [k]$ such that $x_c$ satisfies linear inequalities involving $c_i, d_i$.
In order to encode these constraints as a mixed integer linear programming problem, we introduce $m \times k$ binary variables of the form $w_{l,i} \in \{0, 1\}$ for $l \in [m]$ and  $i \in [k]$. First, we require that for each $l \in [m]$, there must be a corresponding $i \in [k]$:
\begin{equation}\label{eq:psi-1}
\sum_{i=1}^k w_{l, i} \geq 1,\ \text{for}\ l = 1, \ldots, m \,.
\end{equation}
Next, we will encode the constraints involving $c_i$ using the $M$-trick:
\begin{equation}\label{eq:psi-2}
\begin{array}{l}
\hatc_i^t x_c \leq w_{i,l} \hatd_i  + (1-w_{i,l}) M_1 \\ 
(\hatc_i - \hatc_j)^t x_c \geq w_{i,l} (\hatd_i - \hatd_j) + (1 - w_{i,l}) M_2,\ \ \text{for}\ j \in [k] \\ 
(A_l^t \hatc_i + \lambda \hatc_i)^t x_c > w_{i,l} (\lambda \hatd_i - \hatc_i^t b_l)  +(1 - w_{i,l}) M_3 \\ 
\end{array}
\end{equation}

The first constraint encodes the implication that $w_{i,l} = 1$ implies $\hatc_i^t x_c \leq \hatd_i$. The big-M constant $M_1$ is chosen so that $\hatc_i^t x_c \leq M_1$ is true for any choice of $ x_c$.  Likewise, the second constraint ensures that 
whenever $w_{i,l} = 1$, we have $\hatc_i^t x_c - \hatd_i \geq \hatc_j^t x_c - \hatd_j$ for all $j \in [k]$. Similarly, the third constraint enforces the decrease condition with respect to the dynamics $(A_l, b_l)$ for the $i^{th}$ piece of the desired CBF whenever $w_{i,l} =1$. 

Here, $M_1, M_2, M_3$ are constants that are determined by placing an upper bound on the norm $|\vert x_c|\vert_{\infty} \leq M$.  Since, the candidates $(\hat{c}_i, \hatd_i)_{i=1}^k$ is fixed. Let $\alpha = \max_{i=1}^k \|\hatc_i \|_1$. Therefore, we calculate $M_1 = M \alpha$, $M_2 = -2M \alpha$ and  $M_3 = - \alpha (\max_{l=1}^m |\vert A_l|\vert_{\infty} + \lambda)M$. A bound $M$ over the magnitude of $\|x_c\|_{\infty}$ is obtained as follows:

\begin{lem}\label{lem:counterex-big-M-bound}
Let $x_c \in \Real^n$ be a solution to~\eqref{eq:counterex-eq}. Let $\alpha = \max_{i=1}^k \max( \|\hatc_i\|_1, \hatd_i) $ and $U = \max(2, \textcolor{red}{\lambda} + \|A_1 \|_{\infty}, \ldots, \textcolor{red}{\lambda} + \|A_m\|_{\infty} ) \alpha $. It follows that $\|x_c\|_{\infty} \leq (n U)^n$.
\end{lem}
\begin{pf}
Note that by~\eqref{eq:counterex-eq}, there exists a map $\mu: [m] \rightarrow [k]$ and a number $\epsilon > 0 $ such that $x_c$ belongs to a polyhedron defined by inequalities of the form:
\begin{equation}\label{eq:counterex-polyhedral-form} 
\bigwedge_{l=1}^m \left( \begin{array}{c}
\hatc_{\mu(l)} x_c \leq \hatd_{\mu(l)} \\ 
\bigwedge_{j=1}^k (\hatc_{\mu(l)} - \hatc_j)^t x_c \geq \hatd_{\mu(l)} - \hatd_j \\ 
\hatc_{\mu(l)}^t (A_l + \lambda I) x_c \geq \epsilon - \hatc_{\mu(l)}^t b_l + \lambda \hatd_{\mu(l)}
\end{array}\right) 
\end{equation}
A well known result in linear programming (Cf. Bertsimas and Tsitsiklis, Ch. 8~\cite{Bertsimas+Tsitsiklis/1997/Introduction}) states that \textcolor{red}{for any polyhedron $ A x \leq b$, where $x$ is a $n \times 1$ vector of unknowns, if there is a feasible point then there exists a feasible point that satisfies $ \| x \|_{\infty} \leq (n U)^n$,} 
wherein $U$ is the absolute value of the largest entry in $A,b$. The result follows by careful examination of the constraints from~\eqref{eq:counterex-polyhedral-form}. Note that \textcolor{red}{$\|c_i\|_{\infty} \leq \gamma$} and $\|c_j^t (A_l + \lambda I) \|_\infty \leq \|c_j\|_1 ( |\lambda| + \|A_l\|_{\infty})$.
\end{pf}

\begin{thm}
A candidate function $B(x) = \max_{i=1}^k c_i^t x - d_i$ satisfies \textbf{(C3)} if and only if the MILP instance with constraints~\eqref{eq:psi-1} and~\eqref{eq:psi-2} are infeasible for $M$ given by the bound from Lemma~\ref{lem:counterex-big-M-bound}.
\end{thm}

\begin{comment}
%% SRIRAM: Commenting this out. It is deviating from the main thrust of the discussion.
 Although this restricts the space of functions, it is possible to ``compensate'' for this loss by searching for a $k+1$ piece function rather than a function with $k$ pieces. 

\begin{lem}
Suppose $B(x) = \max_{i=1}^k c_i^t x - d_i$ is a polyhedral control barrier function satisfying the conditions in Def.~\ref{def:polyhedral-cbf}. Let $c_{k+1} = \sum_{i=1}^k \lambda_i c_i$ and $d_{k+1} \geq \sum_{i=1}^k \lambda_i d_i$ for multipliers $\lambda_i \geq 0$ satisfying $\sum_{i=1}^k \lambda_i = 1$ and for all $x \in X_u$, $c_{k+1}^t x - d_{k+1} > 0$. The function $\hat{B}(x) = \max_{i=1}^{k+1} c_i^t x - d_i$ is a valid control barrier function.
\end{lem}
\begin{pf}
We will verify that $\hat{B}$ satisfies conditions \textbf{(C1)-(C3)}, starting with \textbf{(C1)}. Let 
$x \in X_0$. We note that $B(x) < 0$: therefore, $c_i^t x - d_i < 0$ for all $i \in [k]$. Hence, $c_{k+1}^t x - d_k \leq \sum_{i=1}^k \lambda_i (c_i^t x - d_i) < 0$. Therefore, $\hat{B}$ satisfies \textbf{(C1)}. Likewise, for all $x$, 
$B(x) \leq \hat{B}(x) $. Therefore, for all $x \in X_u$,
$\hat{B}(x) \geq B(x) > 0$.  $\hat{B}$ satisfies \textbf{(C2)}.  Finally, we verify \textbf{(C3)} holds for $\hat{B}$. 
Let $x$ be such that $B(x) \leq 0$. Also, let $I(x) = \{ i \in [k]\ |\ c_i^t x - d_i = B(x) \}$. Since,  $d_{k+1}  \geq \sum_{i=1}^k \lambda_i d_i$ holds. It follows that $c_{k+1}^t x - d_{k+1} \leq \sum_{i=1}^k \lambda_i (c_i^t x - d_i)$. 
\textbf{(case-1)} Assume that there exists $j \not\in I(x)$ such that $\lambda_j > 0$. It follows that 


\end{pf}

\end{comment}

\subsection{Expanding a Node with a Counterexample}

Suppose the current candidate $(\hat{c}_i, \hat{d}_i)_{i=1}^k \in C(n)$ for a leaf node $n$ of our search tree yields a counterexample $x_c$ as a result of solving~\eqref{eq:counterex-eq}. We discuss the procedure for expanding the node $n$ by adding children $n_1, \ldots, n_j$, wherein $j = k + k \times m$. 

The overall goal is to eliminate all solutions from $C(n)$ that do not satisfy~\eqref{eq:counterex-eq}, \textcolor{blue}{either cause the maximum piece be positive or negative maximum piece that does not hold the decreasing condition}. The set of eliminated solutions will include the candidate solution $(\hatc_i, \hatd_i)_{i=1}^k$, the candidate associated with the node $n$.
\begin{description}
\item[Children \# $1$-$k$:] Note that the  counterexample $x_c$ will no longer apply if $\max_{i=1}^k c_i^t x_c - d_i \geq \epsilon$ for some fixed $\epsilon$.  Therefore, we will create a node $n_i$ for $i \in \{ 1, \ldots, k\}$ wherein $C(n_i) := C(n)\ \land\ (c_i^t x_c - d_i \geq \epsilon  )$.  This yields $k$ children, one for each $i \in [k]$.
\item[Children \# $(k+1)$-$(k+k\times m)$:] For each $i \in [k]$ and $l \in [m]$, we will create a node $n_{i'}$ for  $i' = k\times l + i$ with the constraint:
\[ C(n_{i'}) := \ C(n)\ \land\ \left(
\begin{array}{c}
c_i^t x_c \leq d_{i} - \epsilon \ \land \\
\bigwedge_{j=1}^k c_i^t x_c - d_i \geq c_j^t x_c - d_j \\ 
c_i^t (A_l + \lambda I) x_c \leq \lambda d_i - c_i^t b_l - \epsilon  \\ 
\end{array}\right)\,.\]
Note that $\epsilon > 0$ is a fixed constant. The constraints enforce that $i \in [k]$ is the maximal piece for $B(x)$ at $x = x_c$, that $B(x_c) \leq -\epsilon$ and finally the derivative condition is satisfied ``robustly'' by selecting $l \in [m]$ as the mode for $x = x_c$.  This yields $k \times m$ children, one for each pair $i \in [k]$ and $l \in [m]$. 
\end{description}

\begin{thm}
Let $n_j$ be a child of node $n$ of the tree obtained from a candidate $(c_i, d_i)$ using the process described above. It follows that (a) $C(n_j) \subset C(n)$ and (b) $(\hatc_i, \hatd_i) \not\in C(n_j)$. 
\end{thm}

%% TODO: continue with the proof here. 

